A hierarchical dynamical low-rank algorithm for the stochastic description of large reaction networks

The stochastic description of chemical reaction networks with the kinetic chemical master equation (CME) is important for studying biological cells, but it suffers from the curse of dimensionality: The amount of data to be stored grows exponentially with the number of chemical species and thus exceeds the capacity of common computational devices for realistic problems. Therefore, time-dependent model order reduction techniques such as the dynamical low-rank approximation are desirable. In this paper we propose a dynamical low-rank algorithm for the kinetic CME using binary tree tensor networks. The dimensionality of the problem is reduced in this approach by hierarchically dividing the reaction network into partitions. Only reactions that cross partitions are subject to an approximation error. We demonstrate by two numerical examples (a 5-dimensional lambda phage model and a 20-dimensional reaction cascade) that the proposed method drastically reduces memory consumption and shows improved computational performance and better accuracy compared to a Monte Carlo method.

==> bibliography.tex <==
@article{Albeck_2008,
	author = {Albeck, J. G. and Burke, J. M. and Spencer, S. L. and Lauffenburger, D. A. and Sorger, P. K.},
	doi = {10.1371/journal.pbio.0060299},
	journal = {PLOS Biol.},
	volume = {12},
	number = {6},
	pages = {2831--2852},
	title = {{Modeling a Snap-Action, Variable-Delay Switch Controlling Extrinsic Cell Death}},
	year = {2008}
}

@article{Albi_2022,
	author = {Albi, G. and Chignola, R. and Ferrarese, F.},
	doi = {10.1016/j.matcom.2022.03.019},
	journal = {Math. Comput. Simul.},
	volume = {199},
	pages = {317--340},
	title = {{Efficient ensemble stochastic algorithms for agent-based models with spatial predator--prey dynamics}},
	year = {2022}
}

@article{Anderson_2010,
	author = {Anderson, D. F.},
	doi = {10.1007/s11538-010-9517-4},
	journal = {Bulletin of Mathematical Biology},
	volume = {72},
	pages = {1947--1970},
	title = {{Product-Form Stationary Distributions for Deficiency Zero Chemical Reaction Networks}},
	year = {2010}
}

@article{Arnold_2013,
	author = {Arnold, A. and Jahnke, T.},
	doi = {10.1007/s10543-013-0444-2},
	journal = {BIT Numer. Math.},
	volume = {54},
	pages = {305--341},
	title = {{On the approximation of high-dimensional differential equations in the hierarchical Tucker format}},
	year = {2013}
}

@article{Allmann-Rahn_2022,
	author = {Allmann-Rahn, F. and Grauer, R. and Kormann, K.},
	doi = {10.1016/j.jcp.2022.111562},
	journal = {J. Comput. Phys.},
	volume = {469},
	pages = {111562},
	title = {{A parallel low-rank solver for the six-dimensional Vlasov--Maxwell equations}},
	year = {2022},
}

@article{Barabasi_2009,
	author = {Barab\'{a}si, A.-L.},
	doi = {10.1126/science.1173299},
	journal = {Science},
	volume = {325},
	number = {5939},
	pages = {412--413},
	title = {{Scale-Free Networks: A Decade and Beyond}},
	year = {2009},
}

@article{Cai_2017,
	author = {Cai, X. and Guo, W. and Qiu, J.-M.},
	doi = {10.1007/s10915-017-0554-0},
	journal = {J. Sci. Comput.},
	volume = {73},
	title = {{A high order conservative semi-Lagrangian discontinuous Galerkin method for two-dimensional transport simulations}},
	year = {2017}
}

@article{Cassini_2021,
	author = {Cassini, F. and Einkemmer, L.},
	doi = {10.1016/j.cpc.2022.108489},
	journal = {Comput. Phys. Commun.},
	volume = {280},
	title = {{Efficient 6D Vlasov simulation using the dynamical low-rank framework \texttt{Ensign}}},
	year = {2022}
}

@article{Ceruti_2020,
	author = {Ceruti, G. and Lubich, C. and Walach, H.},
	doi = {10.1137/20M1321838},
	journal = {SIAM J. Numer. Anal.},
	volume = {59},
	number = {1},
	pages = {289--313},
	title = {Time integration of tree tensor networks},
	year = {2021},
}

@article{Ceruti_2022,
	author = {Ceruti, G. and Lubich, C.},
	doi = {10.1007/s10543-021-00873-0},
	journal = {BIT Numer. Math.},
	volume = {62},
	number = {1},
	pages = {23--44},
	title = {{An unconventional robust integrator for dynamical low-rank approximation}},
	year = {2022}
}

@article{Ceruti_2022a,
	author = {Ceruti, G. and Kusch, J. and Lubich, C.},
	doi = {10.1007/s10543-021-00907-7},
	journal = {BIT Numer. Math.},
	volume = {62},
	pages = {1149--1174},
	title = {{A rank-adaptive robust integrator for dynamical low-rank approximation}},
	year = {2022},
}

@article{Ceruti_2023,
	author = {Ceruti, G. and Lubich, C. and Sulz, D.},
	doi = {10.1137/22M1473790},
	journal = {SIAM J. Numer. Anal.},
	volume = {61},
	number = {1},
	pages = {194--222},
	title = {{Rank-adaptive time integration of tree tensor networks}},
	year = {2023}
}

@article{Ceruti_2024,
	author = {Ceruti, G. and Kressner, D. and Sulz, D.},
	doi = {10.48550/arXiv.2405.09952},
	journal = {arXiv},
	title = {{Low-rank Tree Tensor Network Operators for Long-Range Pairwise Interactions}},
	year = {2024}
}

@article{Ceruti_2024a,
	author = {Ceruti, G. and Kusch, J. and Lubich, C.},
	doi = {10.1137/23M1565103},
	journal = {SIAM J. Sci. Comput.},
	volume = {46},
	number = {3},
	pages = {B205--B228},
	title = {{A parallel rank-adaptive integrator for dynamical low-rank approximation}},
	year = {2024}
}

@article{Ceruti_2024b,
	author = {Ceruti, G. and Kusch, J. and Lubich, C.},
	doi = {10.48550/arXiv.2402.08607},
	journal = {arXiv},
	title = {{A robust second-order low-rank BUG integrator based on the midpoint rule}},
	year = {2024}
}

@article{Chen_2010,
	author = {Chen, W. W. and Niepel, M. A. and Sorger, P. K.},
	doi = {10.1101/gad.1945410},
	journal = {Genes Dev.},
	volume = {24},
	number = {17},
	pages = {1861--1875},
	title = {{Classic and contemporary approaches to modeling biochemical reactions}},
	year = {2010}
}

@article{Clarke_2020,
	author = {Clarke, M. A. and Fisher, J.},
	doi = {10.1038/s41568-020-0258-x},
	journal = {Nat. Rev. Cancer},
	volume = {20},
	pages = {343--354},
	title = {{Executable cancer models: successes and challenges}},
	year = {2020}
}

@article{Coughlin_2022,
	author = {Coughlin, J. and Hu, J.},
	doi = {10.1016/j.jcp.2022.111590},
	journal = {J. Comput. Phys.},
	volume = {470},
	pages = {111590},
	title = {{Efficient dynamical low-rank approximation for the Vlasov-Amp\`{e}re-Fokker-Planck system}},
	year = {2022},
}

@article{Ding_2021,
	author = {Ding, Z. and Einkemmer, L. and Li, Q.},
	doi = {10.1137/20M1380788},
	journal = {SIAM J. Numer. Anal.},
	volume = {59},
	number = {4},
	title = {{Dynamical Low-Rank Integrator for the Linear Boltzmann Equation: Error Analysis in the Diffusion Limit}},
	year = {2021}
}

@article{Dinh_2020,
	author = {Dinh, T. and Sidje, R. B.},
	doi = {10.1088/1478-3975/aba1d2},
	journal = {Phys. Biol.},
	volume = {17},
	number = {065014},
	title = {{An adaptive solution to the chemical master equation using quantized tensor trains with sliding windows}},
	year = {2020}
}

@article{Dolgov_2015,
	author = {Dolgov, S. and Khoromskij, B.},
	doi = {10.1002/nla.1942},
	journal = {Numer. Linear Algebra Appl.},
	volume = {22},
	pages = {197--219},
	title = {{Simultaneous state-time approximation of the chemical master equation using tensor product formats}},
	year = {2015}
}

@article{Einkemmer_2018,
	author = {Einkemmer, L. and Lubich, C.},
	doi = {10.1137/18M116383X},
	journal = {SIAM J. Sci. Comput.},
	volume = {40},
	number = {5},
	pages = {B1330--B1360},
	title = {{A Low-Rank Projector-Splitting Integrator for the Vlasov-Poisson Equation}},
	year = {2018}
}

@article{Einkemmer_2020,
	author = {Einkemmer, L. and Ostermann, A. and Piazzola, C.},
	journal = {J. Comput. Phys.},
	volume = {403},
	pages = {109063},
	title = {{A low-rank projector-splitting integrator for the Vlasov--Maxwell equations with divergence correction}},
	year = {2020}
}

@article{Einkemmer_2021,
	author = {Einkemmer, L. and Hu, J. and Wang, Y.},
	doi = {10.1016/j.jcp.2021.110353},
	journal = {J. Comput. Phys.},
	volume = {439},
	number = {110353},
	pages = {110353},
	title = {{An asymptotic-preserving dynamical low-rank method for the multi-scale multi-dimensional linear transport equation}},
	year = {2021}
}

@article{Einkemmer_2021a,
	author = {Einkemmer, L. and Hu, J. and Ying, L.},
	doi = {10.1137/21m1392772},
	journal = {SIAM J. Sci. Comput.},
	volume = {43},
	number = {5},
	pages = {B1057--B1080},
	title = {{An Efficient Dynamical Low-Rank Algorithm for the Boltzmann-{BGK} Equation Close to the Compressible Viscous Flow Regime}},
	year = {2021}
}

@article{Einkemmer_2021b,
	author = {Einkemmer, L. and Joseph, I.},
	doi = {10.1016/j.jcp.2021.110495},
	journal = {J. Comput. Phys.},
	volume = {443},
	pages = {110495},
	title = {{A mass, momentum, and energy conservative dynamical low-rank scheme for the Vlasov equation}},
	year = {2021}
}

@misc{Einkemmer_2021c,
	author = {Einkemmer, L.},
	title = {{Lecture slides: Low-rank approximation for nonlinear kinetic problems -- Part 1: Introduction and the dynamical low-rank algorithm}},
	year = {2021}
}

@article{Einkemmer_2022,
	author = {Einkemmer, L. and Ostermann, A. and Scalone, C.},
	doi = {10.1016/j.jcp.2023.112060},
	journal = {J. Comput. Phys.},
	volume = {484},
	pages = {112060},
	title = {A robust and conservative dynamical low-rank algorithm},
	year = {2023}
}

@article{Einkemmer_2023,
	author = {Einkemmer, L.},
	doi = {10.48550/arXiv.2306.17526},
	journal = {arXiv},
	title = {{Accelerating the simulation of kinetic shear Alfv\'{e}n waves with a dynamical low-rank approximation}},
	year = {2023}
}

@article{Einkemmer_2024,
	author = {Einkemmer, L. and Mangott, J. and Prugger, M.},
	doi = {10.1016/j.jcp.2024.112827},
	journal = {J. Comput. Phys.},
	volume = {503},
	number = {112827},
	title = {{A low-rank complexity reduction algorithm for the high-dimensional kinetic chemical master equation}},
	year = {2024}
}

@article{Einkemmer_2024a,
	author = {Einkemmer, L. and Hu, J. and Kusch, J.},
	doi = {10.1137/23M1547603},
	journal = {SIAM J. Numer. Anal.},
	volume = {62},
	number = {1},
    pages = {73--92},
	title = {Asymptotic--preserving and energy stable dynamical low-rank approximation},
	year = {2024}
}

@article{Engblom_2008,
	author = {Engblom, S.},
	doi = {10.1016/j.cam.2008.10.029},
	journal = {J. Comput. Appl. Math.},
	volume = {229},
	pages = {208--221},
	title = {{Spectral approximation of solutions to the chemical master equation}},
	year = {2008}
}

@book{Erban_2020,
	author = {Erban, R. and Chapman, S. J.},
	doi = {10.1017/9781108628389},
	publisher = {Cambridge University Press},
	title = {{Stochastic Modelling of Reaction--Diffusion Processes}},
	year = {2020}
}

@book{Gardiner_2004,
	author = {Gardiner, C.},
	publisher = {Springer Berlin, Heidelberg},
	title = {{Handbook of Stochastic Methods}},
	year = {2004}
}

@article{Gardner_2000,
	author = {Gardner, T. S. and Cantor, C. R. and Collins, J. J.},
	doi = {10.1038/35002131},
	journal = {Nature},
	volume = {403},
	pages = {339--342},
	title = {{Construction of a genetic toggle switch in \textit{Escherichia coli}}},
	year = {2000}
}

@article{Gaudet_2012,
	author = {Gaudet, S. and Spencer, S. L. and Chen, W. W. and Sorger, P. K.},
	doi = {10.1371/journal.pcbi.1002482},
	journal = {PLOS Comput. Biol.},
	volume = {4},
	number = {8},
	title = {{Exploring the Contextual Sensitivity of Factors that Determine Cell-to-Cell Variability in Receptor-Mediated Apoptosis}},
	year = {2012}
}

@article{Gillespie_1976,
	author = {Gillespie, D. T.},
	doi = {10.1016/0021-9991(76)90041-3},
	journal = {J. Comput. Phys.},
	volume = {22},
	number = {4},
	pages = {403--434},
	title = {{A general method for numerically simulating the stochastic time evolution of coupled chemical reactions}},
	year = {1976}
}

@article{Gillespie_1977,
	author = {Gillespie, D. T.},
	doi = {10.1021/j100540a008},
	journal = {J. Chem. Phys.},
	volume = {81},
	number = {25},
	pages = {2340–-2361},
	title = {{Exact stochastic simulation of coupled chemical reactions}},
	year = {1977}
}

@article{Gillespie_1992,
	author = {Gillespie, D. T.},
	doi = {10.1016/0378-4371(92)90283-V},
	journal = {Physica A},
	volume = {188},
	number = {1},
	pages = {404--425},
	title = {{A rigorous derivation of the chemical master equation}},
	year = {1992}
}

@article{Gillespie_2000,
    author = {Gillespie, D. T.},
    doi = {10.1063/1.481811},
    journal = {J. Chem. Phys.},
    volume = {113},
    pages = {297--306},
    title = "{{The chemical Langevin equation}}",
    year = {2000}
}

@article{Gillespie_2001,
    author = {Gillespie, D. T.},
    doi = {10.1063/1.1378322},
    journal = {J. Chem. Phys.},
    volume = {115},
    number = {4},
    pages = {1716--1733},
    title = "{{Approximate accelerated stochastic simulation of chemically reacting systems}}",
    year = {2001}
}

@article{Grima_2008,
	author = {Grima, R. and Schnell, S.},
	doi = {10.1042/bse0450041},
	journal = {Essays Biochem.},
	volume = {45},
	pages = {41--56},
	title = {{Modelling reaction kinetics inside cells}},
	year = {2008}
}

@misc{Guennebaud_2010,
    author = {Guennebaud, G. and Jacob, B. and others},
    title = {Eigen v3},
    url = {http://eigen.tuxfamily.org},
    year = {2010}
}

@article{Guo_2024,
	author = {Guo, W. and Qiu, J.-M.},
    doi = {10.1137/22M1473960},
	journal = {SIAM J. Sci. Comput.},
    volume = {46},
    number = {1},
    pages = {A232--A263},
	title = {{A conservative low rank tensor method for the Vlasov dynamics}},
	year = {2024}
}

@article{Harris_2006,
	author = {Harris, L. A. and Clancy, P.},
	doi = {10.1063/1.2354085},
	journal = {J. Chem. Phys.},
	volume = {125},
	number = {14},
	title = {A ``partitioned leaping'' approach for multiscale modeling of chemical reaction dynamics},
	year = {2006}
}

@article{Hegland_2007,
	author = {Hegland, M. and Burden, C. and Santoso, L. and MacNamara, S. and Booth, H.},
	doi = {10.1016/j.cam.2006.02.053},
	journal = {J. Comput. Appl. Math.},
	volume = {205},
	pages = {708--724},
	title = {{A solver for the stochastic master equation applied to gene regulatory networks}},
	year = {2007}
}

@article{Hegland_2008,
	author = {Hegland, M. and Hellander, A. and L\"{o}tstedt, P.},
	doi = {10.1007/s10543-008-0174-z},
	journal = {BIT Numer. Math.},
	volume = {48},
	pages = {265--283},
	title = {{Sparse grids and hybrid methods for the chemical master equation}},
	year = {2008}
}

@article{Hegland_2011,
	author = {Hegland, M. and Garcke, J.},
	doi = {10.21914/anziamj.v52i0.3895},
	journal = {ANZIAM J.},
	volume = {52},
	pages = {C628--C643},
	title = {{On the numerical solution of the chemical master equation with sums of rank one tensors}},
	year = {2011}
}

@InProceedings{Henzinger_2009,
    author = {Henzinger, T. A. and Mateescu, M. and Wolf, V.},
    editor = {Bouajjani, A. and Maler, O.},
    doi = {10.1007/978-3-642-02658-4_27},
    volume = {5643},
    pages = {337--352},
    series = {LNTCS},
    booktitle = {{Computer Aided Verification}},
    title = {{Sliding Window Abstraction for Infinite Markov Chains}},
    year = {2009},
    publisher = {Springer}
}

@article{Ion_2021,
	author = {Ion, I. G. and Wildner, C. and Loukrezis, D. and Koeppl, H. and De Gersem, H.},
	doi = {10.1063/5.0045521},
	journal = {J. Chem. Phys.},
	volume = {155},
	number = {034102},
	title = {{Tensor-train approximation of the chemical master equation and its application for parameter inference}},
	year = {2021}
}

@Misc{Jacob_2006,
    author = {Jacob, B. and Guennebaud, G.},
    title = {{Eigen}},
    howpublished = {\url{http://gts.sourceforge.net/}},
    year = {2006--2021}
}

@article{Jahnke_2007,
	author = {Jahnke, T. and Huisinga, W.},
	doi = {10.1007/s00285-006-0034-x},
	journal = {J. Math. Biol.},
	volume = {54},
	pages = {1--26},
	title = {Solving the chemical master equation for monomolecular reaction systems analytically},
	year = {2007}
}

@article{Jahnke_2008,
	author = {Jahnke, T. and Huisinga, W.},
	doi = {10.1007/s11538-008-9346-x},
	journal = {Bull. Math. Biol.},
	volume = {70},
	pages = {2283--2302},
	title = {{A Dynamical Low-Rank Approach to the Chemical Master Equation}},
	year = {2008}
}

@article{Jahnke_2010,
	author = {Jahnke, T. and Udrescu, T.},
	doi = {10.1016/j.jcp.2010.04.015},
	journal = {J. Comput. Phys.},
	volume = {229},
	pages = {5724--5741},
	title = {Solving chemical master equations by adaptive wavelet compression},
	year = {2010}
}

@article{Jahnke_2010a,
	author = {Jahnke, T.},
	doi = {10.1137/080742324},
	journal = {SIAM J. Sci. Comput.},
	volume = {31},
    number = {6},
	pages = {4373--4394},
	title = {An adaptive wavelet method for the chemical master equation},
	year = {2010}
}

@article{VanKampen_1976,
    author = {Van Kampen, N. G.},
    doi = {10.1016/0375-9601(76)90398-4},
    journal = {Phys. Lett. A},
    volume = {59},
    number = {5},
    pages = {333--334},
    title = {{The equilibrium distribution of a chemical mixture}},
    year = {1976}
}

@article{Kazeev_2014,
    author = {Kazeev, V. and Khammash, M. and Nip, M. and Schwab, C.},
    doi = {10.1371/journal.pcbi.1003359},
    journal = {PLOS Comput. Biol.},
    volume = {10},
    number = {3},
    title = {{Direct Solution of the Chemical Master Equation Using Quantized Tensor Trains}},
    year = {2014}
}

@article{Kazeev_2015,
    author = {Kazeev, V. and Schwab, C.},
    doi = {10.1137/130927218},
    journal = {SIAM J. Matrix Anal. Appl.},
    volume = {36},
    number = {3},
    pages = {1221--1247},
    title = {{Tensor approximation of stationary distributions of chemical reaction networks}},
    year = {2015}
}

@article{Koch_2007,
	author = {Koch, O. and Lubich, C.},
	doi = {10.1137/050639703},
	journal = {SIAM J. Matrix Anal. Appl.},
	volume = {29},
	number = {2},
	pages = {434--454},
	title = {{Dynamical Low-Rank Approximation}},
	year = {2007}
}

@article{Kormann_2015,
	author = {Kormann, K.},
	doi = {10.1137/140971270},
	journal = {SIAM J. Sci. Comput.},
	volume = {37},
	pages = {613--632},
	title = {{A semi-Lagrangian Vlasov solver in tensor train format}},
	year = {2015}
}

@article{Kurtz_1972,
	author = {Kurtz, T. G.},
	doi = {10.1063/1.1678692},
	journal = {Journal of Chemical Physics},
	volume = {57},
	pages = {2976--2978},
	title = {{The Relationship between Stochastic and Deterministic Models for Chemical Reactions}},
	year = {1972}
}

@article{Kusch_2021,
	author = {Kusch, J. and Stammer, P.},
	doi = {10.1051/m2an/2022090},
	journal = {ESAIM: Math. Model. Numer. Anal.},
	volume = {57},
	number = {2},
	pages = {865--891},
	title = {{A robust collision source method for rank adaptive dynamical low-rank approximation in radiation therapy}},
	year = {2023}
}

@article{Kusch_2022,
	author = {Kusch, J. and Whewell, B. and McClarren, R. and Frank, M.},
	doi = {10.1016/j.jcp.2022.111587},
	journal = {J. Comput. Phys.},
    volume = {470},
    number = {111587},
	title = {{A low-rank power iteration scheme for neutron transport critically problems}},
	year = {2022}
}

@article{Kusch_2023,
	author = {Kusch, J. and Einkemmer, L. and Ceruti, G.},
	doi = {10.1137/21m1446289},
	journal = {SIAM J. Sci. Comput.},
	volume = {45},
	number = {1},
	pages = {A1--A24},
	title = {{On the Stability of Robust Dynamical Low-Rank Approximations for Hyperbolic Problems}},
	year = {2023}
}

@article{Kusch_2024,
	author = {Kusch, J.},
	doi = {10.48550/arXiv.2403.02834},
	journal = {arXiv},
	title = {{Second-order robust parallel integrators for dynamical low-rank approximation}},
	year = {2024}
}

@article{Lopez_2013,
	author = {Lopez, C. F. and Muhlich, J. L. and Bachman, J. A. and Sorger, P. K.},
	doi = {10.1038/msb.2013.1},
	journal = {Mol. Syst. Biol.},
	volume = {9},
	number = {1},
	pages = {646},
	title = {{Programming biological models in Python using PySB}},
	year = {2013}
}

@book{Lubich_2008,
	author = {Lubich, C.},
	doi = {10.4171/067},
	title = {{From quantum to classical molecular dynamics: reduced models and numerical analysis}},
	year = {2008},
	publisher = {European Mathematical Society}
}

@article{Lubich_2013,
	author = {Lubich, C. and Rohwedder, T. and Schneider, R. and Vandereycken, B.},
	doi = {10.1137/120885723},
	journal = {SIAM J. Matrix Anal. Appl.},
	volume = {34},
	number = {2},
	pages = {470--494},
	title = {Dynamical approximation by hierarchical {T}ucker and tensor-train tensors},
	year = {2013}
}

@article{Lubich_2014,
	author = {Lubich, C. and Oseledets, I. V.},
	doi = {10.1007/s10543-013-0454-0},
	journal = {BIT Numer. Math.},
	volume = {54},
	number = {1},
	pages = {171--188},
	title = {{A projector-splitting integrator for dynamical low-rank approximation}},
	year = {2014}
}

@article{Lubich_2018,
	author = {Lubich, C. and Vandereycken, B. and Walach, H.},
	doi = {10.1137/17M1146889},
	journal = {SIAM J. Numer. Anal.},
	volume = {56},
	number = {3},
	pages = {1273--1290},
	title = {{Time Integration of Rank-Constrained Tucker Tensors}},
	year = {2018}
}

@article{MacNamara_2008,
	author = {MacNamara, S. and Burrage, K. and Sidje, R. B.},
	doi = {10.1137/060678154},
	journal = {SIAM Multiscale Model. Simul.},
	volume = {6},
	number = {4},
	pages = {1146--1168},
	title = {{Multiscale Modeling of Chemical Kinetics via the Master Equation}},
	year = {2008}
}

@article{Matthew_2023,
	author = {Matthew, S. and Carter, F. and Cooper, J. and Dippel, M. and Green, E. and Hodges, S. and Kidwell, M. and Nickerson, D. and Rumsey, B. and Reeve, J. and Petzold, L. R. and Sanft, K. R. and Drawert, B.},
	journal = {Lett. Biomath.},
	volume = {10},
	number = {1},
	pages = {87--103},
	title = {{GillesPy2: A Biochemical Modeling Framework for Simulation Driven Biological Discovery}},
	year = {2023}
}

@article{Meyer_1990,
	author = {Meyer, H.-D. and Manthe, U. and Cederbaum, L. S.},
	doi = {10.1016/0009-2614(90)87014-I},
	journal = {Chem. Phys. Letters},
	volume = {165},
	pages = {73--78},
	title = {The multi-configurational time-dependent {H}artree approach},
	year = {1990},
}

@book{Meyer_2009,
	author = {Meyer, H.-D. and Gatti, F. and Worth, G. A.},
	doi = {10.1002/9783527627400},
	title = {Multidimensional quantum dynamics},
	publisher = {John Wiley \& Sons},
	year = {2009}
}

@article{Munsky_2006,
	author = {Munsky, B. and Khammash, M.},
	doi = {10.1063/1.2145882},
	journal = {J. Chem. Phys.},
	volume = {124},
	number = {4},
	pages = {044104},
	title = {The finite state projection algorithm for the solution of the chemical master equation},
	year = {2006}
}

@article{Niepel_2009,
	author={Niepel, M. and Spencer, S. L. and Sorger, P. K.},
	doi = {10.1016/j.cbpa.2009.09.015},
	volume={13},
	number={5-6},
	pages={556--561},
	title={{Non-genetic cell-to-cell variability and the consequences for pharmacology}},
	journal={Curr. Opin. Chem. Biol.},
	year={2009}
}

@article{Nguyen_2016,
	author = {Nguyen, L. K. and Kholodenko, B. N.},
	doi = {10.1016/j.semcdb.2015.09.024},
	journal = {Seminar in Cell \& Developmental Biology},
	volume = {50},
	pages = {85--94},
	title = {{Feedback regulation in cell signalling: Lessons for cancer therapeutics}},
	year = {2016}
}

@article{Paszek_2010,
	author={Paszek, P. and Ryan, S. and Ashall, L. and Sillitoe, K. and Harper, C. V. and Spiller, D. G. and Rand, D. A. and White, M. R.H.},
	doi = {10.1073/pnas.0913798107},
	journal={PNAS},
	volume={107},
	number={25},
	pages={11644--11649},
	title={{Population robustness arising from cellular heterogeneity}},
	year={2010}
}

@article{Peng_2020,
	author = {Peng, Z. and McClarren, R. and Frank, M.},
	doi = {10.1016/j.jcp.2020.109735},
	journal = {J. Comput. Phys.},
	volume = {421},
	number = {109735},
	title = {{A low-rank method for two-dimensional time-dependent radiation transport calculations}},
	year = {2020}
}

@article{Peng_2021,
	author = {Peng, Z. and McClarren, R.},
	doi = {10.1016/j.jcp.2021.110672},
	journal = {J. Comput. Phys.},
	volume = {447},
	number = {110672},
	title = {{A high-order/low-order (HOLO) algorithm for preserving conservation in time-dependent low-rank transport calculations}},
	year = {2021}
}

@article{Pino_2020,
	author = {Pino, J. C. and Prugger, M. and Lubbock, A. L. R. and Harris, L. A. and Lopez, C. F.},
	doi = {10.1101/2020.02.14.948612},
	journal = {bioRxiv},
	title = {{Accelerated Simulations of Chemical Reaction Systems using the Stochastic Simulation Algorithm on GPUs}},
	year = {2020}
}

@article{Prugger_2023,
	author = {Prugger, M. and Einkemmer, L. and Lopez, C. F.},
	doi = {10.1016/j.jcp.2023.112250},
	journal = {J. Comput. Phys.},
	volume = {489},
	page = {112250},
	title = {{A dynamical low-rank approach to solve the chemical master equation for biological reaction networks}},
	year = {2023}
}

@article{Reis_2018,
	author = {Reis, M. and Kromer, J. A. and Klipp, E.},
	doi = {10.1007/s00285-018-1205-2},
	journal = {J. Math. Biol.},
	volume = {77},
	pages = {377--419},
	title = {General solution of the chemical master equation and modality of marginal distributions for hierarchic first-order reaction networks},
	year = {2018}
}

@article{Saad_1986,
	author = {Saad, Y. and Schultz, M. H.},
	doi = {10.1137/0907058},
	journal = {SIAM J. Sci. Stat. Comput.},
	volume = {7},
	number = {3},
	title = {{GMRES: A generalized minimal residual algorithm for solving nonsymmetric linear systems}},
	year = {1986}
}

@article{Sanft_2011,
	author = {Sanft, K. R. and Wu, S. and Roh, M. and Fu, J. and Lim, R. K. and Petzold, L. R.},
	doi = {10.1093/bioinformatics/btr401},
	journal = {Bioinformatics},
	volume = {27},
	number = {17},
	pages = {2457--2458},
	title = {{StochKit2: software for discrete stochastic simulation of biochemical systems with
events}},
	year = {2011}
}

@article{Sulz_2024,
	author = {Sulz, D. and Lubich, C. and Ceruti, G. and Lesanovsky, I. and Carollo, F.},
	doi = {10.1103/PhysRevA.109.022420},
	journal = {Phys. Rev. A},
	volume = {109},
	number = {022420},
	title = {{Numerical simulation of long-range open quantum many-body dynamics with tree tensor networks}},
	year = {2024}
}

@article{Schloegl_1971,
    author = {Schl\"{o}gl, F.},
    doi = {doi.org/10.1007/BF01395694},
    journal = {Z. Physik},
    volume = {248},
    pages = {446--458},
    title = {On thermodynamics near a steady state},
    year = {1971}
}

@article{Tonn_2019,
	author = {Tonn, M. K. and Thomas, P. and Barahona, M. and Oyarz\'{u}n, D. A.},
	doi = {10.1038/s42003-019-0347-0},
	journal = {Commun. Biol.},
	volume = {2},
	number={108},
	title = {{Stochastic modelling reveals mechanisms of metabolic heterogeneity}},
	year = {2019}
}

@article{Wolf_2010,
	author = {Wolf, V. and Goel, R. and Mateescu, M. and Henzinger, T. A.},
	doi = {10.1186/1752-0509-4-42},
	journal = {BMC Syst. Biol.},
	volume = {4},
	number = {42},
	title = {Solving the chemical master equation using sliding windows},
	year = {2010}
}

@article{Yachie-Kinoshita_2018,
	author = {Yachie-Kinoshita, A. and Onishi, K. and Ostblom, J. and Langley, M. A. and Posfai, E. and Rossant, J. and Zandstra, P. W.},
	doi = {10.15252/msb.20177952},
	journal = {Mol. Syst. Biol.},
	volume = {14},
	number = {1},
	title = {{Modeling signaling-dependent pluripotency with Boolean logic to predict cell fate transitions}},
	year = {2018}
}

@article{Ye_2023,
	author = {Ye, E. and Loureiro, N. F.},
	doi = {10.48550/arXiv.2311.07756},
	journal = {arXiv},
	title = {{Quantized tensor networks for solving the Vlasov--Maxwell equations}},
	year = {2023}
}

@article{Zanudo_2018,
	author = {Za\~{n}udo, J. G. T. and Steinway, S. N. and R\'{e}ka, A.},
	doi = {10.1016/j.coisb.2018.02.002},
	journal = {Curr. Opin. Syst. Biol.},
	volume = {9},
	pages = {1--10},
	title = {{Discrete dynamic network modeling of oncogenic signaling: Mechanistic insights for personalized treatment of cancer}},
	year = {2018}
}
